Multi-student Diffusion Distillation for Better One-step Generators

Diffusion models achieve high-quality sample generation at the cost of a lengthy multistep inference procedure. To overcome this, diffusion distillation techniques produce student generators capable of matching or surpassing the teacher in a single step. However, the student model's inference speed is limited by the size of the teacher architecture, preventing real-time generation for computationally heavy applications. In this work, we introduce Multi-Student Distillation (MSD), a framework to distill a conditional teacher diffusion model into multiple single-step generators. Each student generator is responsible for a subset of the conditioning data, thereby obtaining higher generation quality for the same capacity. MSD trains multiple distilled students, allowing smaller sizes and, therefore, faster inference. Also, MSD offers a lightweight quality boost over single-student distillation with the same architecture. We demonstrate MSD is effective by training multiple same-sized or smaller students on single-step distillation using distribution matching and adversarial distillation techniques. With smaller students, MSD gets competitive results with faster inference for single-step generation. Using 4 same-sized students, MSD significantly outperforms single-student baseline counterparts and achieves remarkable FID scores for one-step image generation: 1.20 on ImageNet-64x64 and 8.20 on zero-shot COCO2014.

==> sections/abstract.tex <==
% \vspace{-0.02\textheight}
\begin{abstract}
% \vspace{-0.01\textheight}
% Diffusion models generates realistic images with an expensive multi-step denoising process. Recent works uses distillation techniques to train student generators capable of matching/surpassing the teacher performance, with as few as a single forward step. However, most of these works focuses on distilling into a single student with the same architecture and input condition set. We introduce \LongMethodName~(\ShortMethodName), a framework that allows distilling a conditional teacher diffusion model into multiple single step generators. \ShortMethodName{} partitions the conditional input sets into subsets, which are used to distill the same teacher into different students. \ShortMethodName{} comes with flexible dataset partitioning and filtering choices, which together offers a plug-and-play upgrade to the distilled model capability without incuring additional training cost or inference latency.  We demonstrate the effectiveness of \ShortMethodName{} by training $4$ students using Distribution Matching Distillation (DMD) and DMD2 procedures, which sets new benchmarks on one-step image generation: FID $1.14$ on ImageNet-64$\times$64 and $??$ on zero-shot COCO 2014. In addition, by introducing an additional pretraining stage, we successfully distill the teacher into a smaller specialized student with randomly initialized weight, and achieved competitive FID score on a subset of ImageNet classes. Together with \ShortMethodName{}, we demonstrate the promising direction of further improving the generation speed with multiple smaller students.
% \Yanke{Sentences of previous abstract commented.}
% \Weili{It seems the format is still not right: We are missing the "Abstract" title.} 
Diffusion models achieve high-quality sample generation at the cost of a lengthy multistep inference procedure.
To overcome this, diffusion distillation techniques produce student generators capable of matching or surpassing the teacher in a single step.
However, the student model's inference speed is limited by the size of the teacher architecture, preventing real-time generation for computationally heavy applications.
% applications like video synthesis.
% However, the student models use the same architecture as the teacher, which limits their capacity and prevents real-time generation for applications like video synthesis due to the teacher size\James{Need to refine the prior sentence.}.
In this work, we introduce \LongMethodName{} (\ShortMethodName{}), a framework to distill a conditional teacher diffusion model into multiple single-step generators. Each student generator is responsible for a subset of the conditioning data, thereby obtaining higher generation quality for the same capacity. 
\ShortMethodName{} trains multiple distilled students allowing smaller sizes and, therefore, faster inference.
Also, MSD offers a lightweight quality boost over single-student distillation with the same architecture.
We demonstrate \ShortMethodName{} is effective by training multiple same-sized or smaller students on single-step distillation using distribution matching and adversarial distillation techniques. With smaller students, \ShortMethodName{} gets competitive results with faster inference for single-step generation. 
Using $4$ same-sized students, \ShortMethodName{} sets a new state-of-the-art for one-step image generation: FID $1.20$ on ImageNet-64$\times$64 and \FIDSDADM{} on zero-shot COCO2014.
% \ShortMethodName{} unlocks potentials for accelerating diffusion models beyond the step reduction.
% Further, we successfully distill the teacher into smaller specialized students to reduce training cost and achieve extremely fast generation (X\emph{ms}) without compromising quality.
% \James{Touting real-time video generation here would be really nice...}
% \Yanke{Remove the last sentence. Change the order of last two sentences.}
\end{abstract}
% \vspace{-0.02\textheight}

==> sections/conclusion.tex <==
\vspace{-0.01\textheight}
\section{Discussion}
\vspace{-0.01\textheight}
\subsection{Limitations}
\ShortMethodName{} is the first work to explore diffusion distillation with multiple students, and it admits a few limitations that call for future work.
1) Further explorations could offer more insights into optimal design choices for a target quality and latency on various datasets, such as the number of students, input condition size for each student, and other hyperparameters. This is especially beneficial if the training budget is limited. 2) We apply simple partitioning for both class- and text-conditions and assign them disjointly to different students. Although our empirical study shows that simple alternatives do not offer obvious advantages, more sophisticated routing mechanisms may help. 3) We use simple channel reduction when designing smaller students to demonstrate feasibility. This results in a significantly smaller latency reduction than sample size reduction.
Exploring other designs of smaller students will likely increase their quality and throughput.
4) We train different students separately, but we expect that carefully designed weight-sharing, loss-sharing, or other interaction schemes can further enhance training efficiency. 5) We hypothesize that \ShortMethodName{} can be applied to other diffusion distillation methods and other modalities for similar benefits, but leave this for future work.
% \Jon{This paragraph feels pretty weak atm, but unclear how much we want to put here for conference submission. Would be good to clearly go through each part of our method one-by-one and discuss limitations for each component.  Unclear how much we want to elaborate on limitations for conference, but for arXiv I think expanding on limitations with respect to each part of our results (a) clustering, (b) choice of distillation method, (c) training methodology, (d) compute budget for experiments, (e) modalities, (f) smaller architecture choices, (g) hyperparameter choices, (h) using ultra-large teacher models, ... would be useful to readers.}
\vspace{-0.01\textheight}
\subsection{Conclusion}
This work presented \LongMethodName{}, a simple yet efficient method to increase the effective model capacity for single-step diffusion distillation. We applied \ShortMethodName{} to the distribution matching and adversarial distillation methods. We demonstrated their superior performance over single-student counterparts in both class-conditional generation and text-to-image generation. Particularly, \ShortMethodName{} with DMD2's the two-stage training achieves state-of-the-art FID scores. Moreover, we successfully distilled smaller students from scratch, demonstrating \ShortMethodName{}'s potential in further reducing the generation latency with multiple smaller student distillations. We envision building on \ShortMethodName{} to enable generation in real-time, enabling many new use cases.


==> sections/experiments/2d.tex <==
\subsection{Toy Experiments}\label{subsec:toy}
In Fig.~\ref{fig:2d}, we show the sample density of \ShortMethodName{} with \StageOneName{} stage for a 2D toy experiment, where the real data distribution has $8$ classes, and each class is a mixture of $8$ Gaussians.
We used a simple MLP with EDM schedules to train the teacher and then distill into $1$, $2$, $4$, and $8$ students for comparison.
From the displayed samples and the $\ell_1$ distance from teacher generation, we observe that the collective generation quality increases as the number of students increases.




==> sections/experiments/ablation.tex <==
\vspace{-0.01\textheight}
\subsection{Ablation Studies}\label{subsec:ablation}

Here, we ablate the effect of different components in \ShortMethodName{} and offer insight into scaling. Unless otherwise mentioned, all experiments are conducted for class-conditional generation ImageNet-64$\times$64, using only the \StageOneName{} stage for computational efficiency.

\textbf{\ShortMethodName{} is still better with the same effective batch size.} 
% \James{We could include the table you made before that has batch size (in the appendix). We can point out that batch size is a critical variable for diffusion distillation. So, we wanted to validate that our method is useful without an effective batch size increase due to multiple students.} 
To investigate if the performance boost from \ShortMethodName{} comes from only a batch size increase over single student distillation, we make a comparison with the same effective batch size. As showcased in Tab.~\ref{tab:ablation}, MSD with $4$ students and a batch size of $32$ per student performs slightly better than the single-student counterpart with a batch size of $128$, indicating that \ShortMethodName{} likely benefits from a capacity increase than a batch size increase.
As a takeaway, with a fixed training resource measured in processed data points, users are better off distilling into multiple students with partitioned resources each than using all resources to distill into a single student. This is also reflected in our previous experiments, where we used significantly less resources per student than the single-student counterparts (see details in App.~\ref{sec:implementation}). Although multiple students means multiple model weights to save, storage is often cheap, so in many applications, this cost is outweighed by our improved quality or latency.

\begin{wraptable}[14]{r}{0.48\textwidth}
\centering
\vspace{-0.25cm}
\caption{Ablation studies on different components of MSD. All experiments are done on ImageNet-64$\times$64, trained with only the DM stage for $20$k iterations, where $B$ is the batch size per student. See App. \ref{subsec:ablation_curve}.}
\scalebox{0.85}{
\begin{tabular}{l c} 
\hline 
Method & FID ($\downarrow$)\\ 
\hline 
{$4$ students, $B=32$} & \num{2.53}\\
{$1$ students, $B=128$} & \num{2.60}\\
{$2$ students, $B=128$} & \num{2.49}\\
\textbf{$\bf{4}$ students, $\bf{B=128}$ (baseline)} & \num{2.37}\\
{$8$ students, $B=128$} & \num{2.32}\\
{$4$ students, $B=128$, $K$-means splitting} & \num{2.39}\\
{$4$ students, $B=128$, random splitting} & \num{2.45}\\
\hline
\end{tabular}
}
\label{tab:ablation}
\end{wraptable}

\textbf{Simple splitting works surprisingly well.} We used consecutive splitting of classes in Sec.~ \ref{subsec:imagenet}. Although it shows obvious advantage over random splitting, as shown in Tab.~\ref{tab:ablation}, it does not use the embedding information from the pretrained EDM model. Therefore, we investigated another strategy where we performed a $K$-means clustering ($K = 4$) on the label embeddings, resulting in $4$ clusters of similar sizes: $(230, 283, 280, 207)$. However, \ShortMethodName{} trained with these clustered partitions performs similarly to sequential partition, as shown in Tab.~\ref{tab:ablation}. For text-to-image generation, we performed $K$-means clustering on the pooled embeddings of prompts in the training data, resulting in clusters of vastly uneven sizes. Due to computational limitations, we opted for the simpler partition strategies outlined in Sec.~\ref{sec:experiments}.

\textbf{Effect of scaling the number of students.} In Tab.~\ref{tab:ablation}, we study the effect of increasing $K$, the number of distilled students. We kept the per-student batch size fixed so more students induce a larger effective batch size. We observe better FID scores for more students. We hypothesize that better training strategies, such as per-student tuning, will further improve the quality. Optimal strategies for scaling to ultra-large numbers of students is an interesting area for future work.


==> sections/experiments/ccond.tex <==
\subsection{Class-conditional Image Generation}\label{subsec:imagenet}

\textbf{Student architecture the same as the teacher:}
We trained $K = 4$ students using the \ShortMethodName{} framework and the EDM \citep{karras2022elucidating} teacher on class-conditional ImageNet-64$\times$64 generation. We applied the simplest strategy for splitting classes among students: Each student is responsible for $250$ consecutive classes in numerical order (i.e., $\nicefrac{1}{K}$ of the $1000$ classes). We compare the performance with previous methods and display the results in Tab.~\ref{tab:imagenet_short}. Our \StageOneName{} stage, which uses the complementary regression loss, surpasses the one-student counterpart DMD \citep{yin2024one}, achieving a modest drop of $\num{0.25}$ in FID score, making it a strong competitor in single-step distillation without an adversarial loss. We then took the best pretrained checkpoints and trained with the \StageTwoName{} stage. The resulting model achieved the current state-of-the-art FID score of $\num{1.20}$. It surpasses even the EDM teacher, StyleGAN-XL \citep{sauer2022styleganxl}, the multi-step RIN \citep{jabri2023scalable} due to the adversarial loss. Fig.~\ref{fig:imagenet_scratch_comparison}(a) and (b) display a comparison of sample generations, showing that our best students have comparable generation quality as the teacher.

\begin{table}[t]
\centering
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \captionsetup{type=table}
    \caption{Comparing
    class-conditional generators on ImageNet-64$\times$64. The number of function evaluations (NFE) for \ShortMethodName{} is $\num{1}$ as a single student is used at inference for the given input.
}
    \scalebox{0.7}{
    \begin{tabular}{l c c} 
    \hline 
    Method & NFE ($\downarrow$) & FID ($\downarrow$)\\ 
    \hline 
    \textit{Multiple Steps}\\
    RIN \citep{jabri2023scalable} & $\num{1000}$ & \num{1.23}\\
    ADM \citep{dhariwal2021diffusion} & $\num{250}$ & \num{2.07}\\
    DPM Solver \citep{lu2022dpm} & \num{10} & \num{7.93}\\
    Multistep CD \citep{heek2024multistep} & \num{2} & \num{2.0}\\
    \hline
    \textit{Single Step, w/o GAN}\\
    PD \citep{salimans2022progressive} & \num{1} & \num{15.39}\\
    DSNO~\citep{zheng2023fast} & \num{1} & \num{7.83} \\
    Diff-Instruct \citep{luo2024diff} & \num{1} & \num{5.57}\\
    iCT-deep \citep{song2023improved} & \num{1} & \num{3.25}\\
    Moment Matching \citep{salimans2024multistep} & \num{1} & \num{3.0}\\
    DMD \citep{yin2024one} & \num{1} & \num{2.62}\\
    \textbf{\ShortMethodName{} (ours): 4 students, \StageOneName{} only} & \num{1} & \num{2.37}\\
    EMD \citep{xie2024distillation} & \num{1} & \num{2.20}\\
    SiD \citep{zhou2024score} & \num{1} & \num{1.52}\\
    \hline
    \textit{Single Step, w/ GAN}\\
    Post-distillation, 4, 42\% smaller students & \num{1} & \num{11.67}\\
    \textbf{\ShortMethodName{} (ours): 4, 42\% smaller students, \StageTwoName{}} & \num{1} & \FIDIADMS\\
    StyleGAN-XL \citep{sauer2022styleganxl} & \num{1} & \num{1.52}\\
    CTM \citep{kim2023consistency} & \num{1} & \num{1.92}\\
    DMD2 \citep{yin2024improved} & \num{1} & \num{1.28}\\
    \textbf{\ShortMethodName{} (ours): 4 students, \StageTwoName{}} & \num{1} & \num{1.20}\\
    \hline 
    \textit{teacher}\\
    EDM (teacher, ODE) \citep{karras2022elucidating} & \num{511} & \num{2.32}\\
    EDM (teacher, SDE) \citep{karras2022elucidating} & \num{511} & \num{1.36}\\
    \hline
    \end{tabular}
    }
    \label{tab:imagenet_short}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\linewidth}
\centering
\captionsetup{type=table}
\caption{Comparing \ShortMethodName{} to other methods on zero-shot text-to-image generation on MS-COCO2014. We measure speed with sampling time per prompt (latency) and quality with FID. 
}
\scalebox{0.7}{
    \begin{tabular}{l c c} 
    \hline 
    Method & Latency ($\downarrow$) & FID ($\downarrow$)\\ 
    \hline 
    \textit{Unaccelerated}\\
    DALL$\cdot$E 2 \citep{ramesh2022hierarchical} & - & $\num{10.39}$\\
    LDM \citep{rombach2022high} & \num{3.7}s & \num{12.63}\\
    eDiff-I \citep{balaji2022ediff} & \num{32.0}s & \num{6.95}\\
    \hline
    \textit{GANs}\\
    StyleGAN-T \citep{sauer2023stylegant} & \num{0.10}s & \num{12.90}\\
    GigaGAN \citep{yu2022scaling}  & \num{0.13}s & \num{9.09}\\
    \hline
    \textit{Accelerated}\\
    DPM++ (4 step) \citep{lu2022dpmp} & \num{0.26}s & \num{22.36}\\
    InstaFlow-0.9B \citep{liu2023instaflow} & \num{0.09}s & \num{12.10}\\
    UFOGen \citep{xu2024ufogen} & \num{0.09}s & \num{12.78}\\
    DMD \citep{yin2024one} & \num{0.09}s & \num{11.49}\\
    EMD \citep{xie2024distillation} & \num{0.09}s & \num{9.66}\\
    DMD2 (w/o GAN) & \num{0.09}s & \num{9.28}\\
    \textbf{\ShortMethodName{} (ours): 4 students, \StageOneName{} only} & \num{0.09}s & \num{8.80}\\
    DMD2 \citep{yin2024improved} & \num{0.09}s & \num{8.35}\\
    \textbf{\ShortMethodName{} (ours): 4 students, \StageTwoName{}} & \num{0.09}s & \FIDSDADM\\
    \hline 
    \textit{teacher}\\
    SDv1.5 ($50$ step, CFG=3, ODE)  & \num{2.59}s & \num{8.59}\\
    SDv1.5 ($200$ step, CFG=2, SDE)  & \num{10.25}s & \num{7.21}\\
    \hline
    \end{tabular}
    }
\label{tab:sd_short}
\end{minipage}
\vspace{-0.02\textheight}
\end{table}


\textbf{Student architecture smaller than the teacher:}
Next, we trained $4$ smaller student models with the prepended teacher score matching (\StageZeroName{}) stage from Sec.~\ref{subsec:from_scratch}. This achieved a $42\%$ reduction in model size and a $7\%$ reduction in latency, with a slight degradation in FID score, offering a flexible framework to increase generation speed by reducing student size, and increasing generation quality by training more students.
Fig.~\ref{fig:imagenet_scratch_comparison}(c) displays sample generation from these smaller students, whereas Fig.~\ref{fig:imagenet_scratch_comparison}(d) shows sample generations from an even smaller set of students, with a $71\%$ percent reduction in model size and a $23\%$ percent reduction in latency. We observed slightly degraded but still competitive generation qualities. Using more and larger students will further boost performance, as shown by ablations in Sec.~\ref{subsec:ablation} and App.~\ref{subsec:smaller_students_comparison}. Smaller students without the \StageZeroName{} stage fail to reach even proper convergence. Moreover, instead of the TSM stage, we performed post output distillation on best single-step checkpoints, and observed significant drop in performance. Hence the TSM stage is both necessary and efficient.
% \James{Last two sentences unclear, do we do these experiments? ``We leave those''}



\begin{figure}[ht]
    \vspace{-0.02\textheight}
    \begin{tikzpicture}[scale=0.7, every node/.style={anchor=west}]
        % Original images
        \node (img11) at (0,0) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.23\linewidth]{plots/imagenet_conparison_teacher.pdf}};
        \node [right=of img11, xshift=-0.9cm] (img12) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.23\linewidth]{plots/imagenet_conparison_baseline.pdf}};
        \node [right=of img12, xshift=-0.9cm] (img13) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.23\linewidth]{plots/imagenet_conparison_scratch1.pdf}};
        \node [right=of img13, xshift=-0.9cm] (img14) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.23\linewidth]{plots/imagenet_conparison_scratch2.pdf}};

        \node[below=of img11, node distance=0cm, yshift=1.1cm, font=\color{black}] {(a) Teacher (multistep)};
        \node[below=of img12, node distance=0cm, yshift=1.1cm, font=\color{black}] {(b) Same-sized students};
        \node[below=of img13, node distance=0cm, yshift=1.1cm, font=\color{black}] {(c) 42\% smaller students};
        \node[below=of img14, node distance=0cm, yshift=1.1cm, font=\color{black}] {(d) 71\% smaller students};
    \end{tikzpicture}
    \vspace{-0.03\textheight}
    \caption{Sample generations on ImageNet-64$\times$64 from the teacher and different sized students, with architecture and latency details in App.~\ref{sec:implementation}. The same-size students have comparable or slightly better generation quality than the teacher. Smaller students achieve faster generation while still having decent qualities. Same-sized students are trained with \StageOneName{} and \StageTwoName{} stages, whereas smaller students are trained with all three stages (see Fig.~\ref{fig:three-stage_training}).
    % \Jon{Where is the latency for the smaller students listed? I would re-iterate it here, and include in tables above perhaps.}
    }
    \label{fig:imagenet_scratch_comparison}
    % \vspace{-0.01\textheight}
\end{figure}

\begin{figure}[ht]
    \vspace{-0.01\textheight}
    \begin{tikzpicture}[scale=0.7, every node/.style={anchor=west}]
        % Original images
        \node (img11) at (0,0) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.31\linewidth]{plots/SD_dog_comparison_teacher.pdf}};
        \node [right=of img11, xshift=-0.9cm] (img12) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.31\linewidth]{plots/SD_dog_comparison_baseline.pdf}};
        \node [right=of img12, xshift=-0.9cm] (img13) {\includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=.31\linewidth]{plots/SD_dog_comparison_scratch_GAN_finetune.pdf}};

        \node[below=of img11, node distance=0cm, yshift=1.1cm, font=\color{black}] {(a) Teacher (multistep)};
        \node[below=of img12, node distance=0cm, yshift=1.1cm, font=\color{black}] {(b) Same-sized student};
        \node[below=of img13, node distance=0cm, yshift=1.1cm, font=\color{black}] {(c) 83\% smaller student};
    \end{tikzpicture}
    \caption{Samples on high guidance-scale text-to-image generations from the SD v1.5 teacher and different sized students, with full training details in App.~\ref{sec:implementation}. The same-sized student has comparable quality to the teacher. The smaller student, trained on a subset of dog-related data, achieves faster generation while still having decent qualities. The same-sized student is trained with \StageOneName{} stage only, whereas the smaller student is trained with \StageZeroName{} and \StageOneName{} stages (see Fig.~\ref{fig:three-stage_training}).
    % \Jon{Where is the latency for the smaller students listed? I would re-iterate it here, and include in tables above perhaps.}
    }
    \label{fig:SD_scratch_comparison}
    \vspace{-0.02\textheight}
\end{figure}

==> sections/experiments/experiments.tex <==
\section{Experiments}\label{sec:experiments}
\begin{figure}[t]
    \vspace{-0.02\textheight}
    \centering
    \begin{tikzpicture}[scale=0.7, every node/.style={anchor=west}]
        % Original images
        \node (img11) at (0,0) {\includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm}, clip, width=.23\linewidth]{plots/2d_smallsigma_hist_teacher.pdf}};
        \node [right=of img11, xshift=-0.9cm] (img12) {\includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm}, clip, width=.23\linewidth]{plots/2d_smallsigma_hist_single.pdf}};
        \node [right=of img12, xshift=-0.9cm] (img13) {\includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm}, clip, width=.23\linewidth]{plots/2d_smallsigma_hist_8.pdf}};
        \node [right=of img13, xshift=-0.555cm] (img14) {\includegraphics[trim={0.0cm 0.0cm 0.0cm 0.0cm}, clip, width=.23\linewidth]{plots/toy_2d.pdf}};
        
        % Original labels
        \node[left=of img14, rotate=90, anchor=center, yshift=-1.0cm] {$\ell_1$ distance};
        \node[below=of img11, node distance=0cm, yshift=1.1cm, font=\color{black}] {Teacher};
        \node[below=of img12, node distance=0cm, yshift=1.1cm, font=\color{black}] {1 student};
        \node[below=of img13, node distance=0cm, yshift=1.1cm, font=\color{black}] {8 students};
        \node[below=of img14, node distance=0cm, yshift=1.1cm, font=\color{black}] {Number of students};
        
        \begin{scope}  
            \node[draw=black, thin, inner sep=0pt, minimum width=0.7cm, minimum height=0.7cm] (box1) at ($(img11.north west) + (1.23cm, -0.70cm)$) {};
        \end{scope}
        \begin{scope}  
            \node[draw=black, thin, inner sep=0pt, minimum width=0.7cm, minimum height=0.7cm] (box2) at ($(img12.north west) + (1.23cm, -0.70cm)$) {};
        \end{scope}
        \begin{scope}  
            \node[draw=black, thin, inner sep=0pt, minimum width=0.7cm, minimum height=0.7cm] (box3) at ($(img13.north west) + (1.23cm, -0.70cm)$) {};
        \end{scope}
        

        \node[draw=black, thick, inner sep=0pt, minimum width=1.0cm, minimum height=1.0] (zoom1) at ($(img11.north west) + (1.4cm, -2.5cm)$) {
            \begin{tikzpicture}
                % Include the same image, scaled up
                \node at (1.25cm, -4.0cm) {\includegraphics[trim={2.85cm 7.5cm 5.6cm 0.85cm}, clip, width=1.5cm]{plots/2d_smallsigma_hist_teacher.pdf}};
            \end{tikzpicture}
        };
        \node[draw=black, thick, inner sep=0pt, minimum width=1.0cm, minimum height=1.0] (zoom2) at ($(img12.north west) + (1.4cm, -2.5cm)$) {
            \begin{tikzpicture}
                % Include the same image, scaled up
                \node at (1.25cm, -4.0cm) {\includegraphics[trim={2.85cm 7.5cm 5.6cm 0.85cm}, clip, width=1.5cm]{plots/2d_smallsigma_hist_single.pdf}};
            \end{tikzpicture}
        };
        \node[draw=black, thick, inner sep=0pt, minimum width=1.0cm, minimum height=1.0] (zoom3) at ($(img13.north west) + (1.4cm, -2.5cm)$) {
            \begin{tikzpicture}
                % Include the same image, scaled up
                \node at (1.25cm, -4.0cm) {\includegraphics[trim={2.85cm 7.5cm 5.6cm 0.85cm}, clip, width=1.5cm]{plots/2d_smallsigma_hist_8.pdf}};
            \end{tikzpicture}
        };
        
        
        % Draw a bunch of lines
        \begin{scope} %[on background layer]
            \draw[gray, thin, dashed] (box1.south west) -- (zoom1.south west);
            \draw[gray, thin, dashed] (box1.south east) -- (zoom1.south east);
            \draw[gray, thin, dashed] (box1.north west) -- (zoom1.north west);
            \draw[gray, thin, dashed] (box1.north east) -- (zoom1.north east);
            \draw[gray, thin, dashed] (box2.south west) -- (zoom2.south west);
            \draw[gray, thin, dashed] (box2.south east) -- (zoom2.south east);
            \draw[gray, thin, dashed] (box2.north west) -- (zoom2.north west);
            \draw[gray, thin, dashed] (box2.north east) -- (zoom2.north east);
            \draw[gray, thin, dashed] (box3.south west) -- (zoom3.south west);
            \draw[gray, thin, dashed] (box3.south east) -- (zoom3.south east);
            \draw[gray, thin, dashed] (box3.north west) -- (zoom3.north west);
            \draw[gray, thin, dashed] (box3.north east) -- (zoom3.north east);
        \end{scope}

    \end{tikzpicture}
    \caption{
        A 2D toy model.
        From left to right: teacher (multi-step) generation and student, one-step generation with $1$ and $8$ distilled students, the $\ell_1$ distance of generated samples between teacher and students.
        \textbf{Takeaway:} More students improve distillation quality on this easy-to-visualize setup.
        % The mean absolute difference of histogram binned values from the teacher generation approximates the $\ell_1$ distance.
        % \Jon{Took a stab at zooming into a cluster - can probably be refined}
        % \Jon{Can you boost font size in your figure so numbers are about the same size as the main text? Also, saying "distance value" sounds awkward in axis (but your prior explanation makes sense). Can you say something more direct in the axis label, like perhaps "loss on ground Truth" or "divergence between generated and true"?}
        % \James{I'm curious about what happens with more students. Is it easy to extend the graph to 16,32,64 students by splitting up the intra-cluster modes?}\Yanke{not very easy. I only gave 8 labels, so need to retrain everything if we want more splits.}\James{Let's keep it as-is then!}
        % \Yanke{some more style tweak}
    }
    \label{fig:2d}
    \vspace{-0.015\textheight}
\end{figure}

To evaluate the effectiveness of our approach, we trained \ShortMethodName{} with different design choices and compared against competing methods, including other single-step distillation methods.

In Sec.~\ref{subsec:toy}, we compare single vs multiple students on a 2D toy problem for direct visual comparison. For these experiments, we used only the \StageOneName{} stage. In Sec.~\ref{subsec:imagenet}, we investigate class-conditional image generation on ImageNet-64$\times$64 \citep{deng2009imagenet} where we have naturally defined classes to partition. Here we explored training with the \StageOneName{} stage only, with both \StageOneName{} and \StageTwoName{} stages, and with all three stages for smaller students. We then evaluate MSD for a larger model in Sec.~\ref{subsec:t2i}. We explored text-to-image generation on MS-COCO2014 \citep{lin2014microsoft} with varying training stages.
We use the standard Fr\'{e}chet Inception Distance (FID) \citep{heusel2017gans} score to measure generation quality. Comprehensive comparisons confirm that MSD outperforms single-student counterparts and achieves state-of-the-art performance in single-step diffusion distillation. 
Finally, in Sec.~\ref{subsec:ablation}, we summarize our ablation experiments over design choices.

To focus on the performance boost from multi-student distillation, we applied minimal changes to the hyperparameters used by \citet{yin2024one,yin2024improved} for their distribution matching distillation implementations. More details on training and evaluation can be found in the App.~\ref{sec:implementation} and \ref{sec:evaluation}.



\input{sections/experiments/2d}
\input{sections/experiments/ccond}
\input{sections/experiments/t2im}
\input{sections/experiments/ablation}





==> sections/experiments/t2im.tex <==
\vspace{-0.01\textheight}
\subsection{Text-to-Image Generation}\label{subsec:t2i}
\textbf{Student architecture the same as the teacher:} We evaluated the performance of text-to-image generation using the MS-COCO2014 \citep{lin2014microsoft} evaluation dataset. We distilled $4$ students from Stable Diffusion (SD) v1.5 \citep{rombach2022high} on a 5M-image subset of the COYO dataset \citep{kakaobrain2022coyo-700m}. For splitting prompts among students, we again employed a minimalist design: pass the prompts through the pre-trained SD v1.5 text encoder, pool the embeddings over the temporal dimension, and divide into $4$ disjoint subsets along $4$ quadrants. We trained with a classifier-free guidance (CFG) scale of $1.75$ for best FID performance. Tab.~\ref{tab:sd_short} compares the evaluation results with previous methods. Our baseline method with only the \StageOneName{} stage again achieved a performance boost with a $\num{0.48}$ drop in FID over the single-student counterpart DMD2 without adversarial loss \citep{yin2024improved}. Continuing the \StageTwoName{} stage from the best checkpoint yielded a terminal FID of \FIDSDADM, again surpassing the single-student counterpart and achieving the current state-of-the-art FID score. In addition, for better visual quality, we also train with a larger CFG scale of $8$, and display corresponding samples in Fig.~\ref{fig:SD_scratch_comparison}(b) and App.~\ref{subsec:qualitative_SD}.

\textbf{Student architecture smaller than the teacher:} As a preliminary exploration, with the prepended teacher score matching (\StageZeroName{}) stage, we train a $83\%$ smaller and $5\%$ faster student on a dog-related prompt subset of COYO (containing $\sim \num{1210000}$ prompts). We trained with a CFG scale of $8$ and display the samples in Fig.~\ref{fig:SD_scratch_comparison}. We observed fair generation quality despite a significant drop in model size. Improved training is likely to obtain better sample quality and generalization power. Due to limited computational resources and the complete coverage of the prompt set by the 4-student model, we did not train the full set of students at this size.


==> sections/intro.tex <==
\section{Introduction}
% \vspace{-0.01\textheight}
\label{sec:introduction}
% \Yanke{TODOs: 2) Update figure 1} 
Diffusion models are the dominant generative model in image, audio, video, 3D assets, protein design, and more \citep{ho2020denoising, kong2020diffwave, blattmann2023align, anand2022protein, nichol2022point}. They allow different conditioning inputs -- such as class labels, text, or images -- and achieve high-quality generated outputs. However, their inference process typically requires hundreds of model evaluations -- with an often slow and bulky network -- for a single sample. This procedure costs millions of dollars per day \citep{website_numbers, website_costper}. It also prohibits applications requiring rapid synthesis, such as augmented reality. Real-time, low-cost, and high-quality generation will have huge financial and operational impacts while enabling new usage paradigms.

There has been a flurry of work on diffusion-distillation techniques to address the slow sampling of diffusion models \citep{luhman2021knowledge, song2023consistency, yin2024one}. Inspired by knowledge distillation \citep{hinton2015distilling}, these methods use the trained diffusion model as a teacher and optimize a student model to match its generated output in as few as a single step. However, most diffusion distillation methods use the same student and teacher architecture. This prevents real-time generation for applications with bulky networks, such as video synthesis \citep{blattmann2023align}. 
While reducing model size can reduce inference time, it typically yields worse generation quality, thus presenting a speed-to-quality tradeoff dilemma with existing distillation methods.

We tackle this dilemma with our method, \LongMethodName{} (\ShortMethodName{}), that introduces multiple single-step student generators distilled from the pretrained teacher. Each student is responsible for a subset of conditioning inputs.
We determine which student to use during inference and perform a single-model evaluation to generate a high-quality sample. This way, \ShortMethodName{} enjoys the benefit of a mixture of experts \citep{jordan1994hierarchical}: it increases the model capacity without incurring more inference cost, thereby effectively pushing the limit of the speed-quality tradeoff.

When distilling into the same-sized students, \ShortMethodName{} has the flexibility of being conceptually applicable to any distillation method for a performance boost. In addition, \ShortMethodName{} allows distilling into multiple smaller students for reduced single-step generation time. Using smaller students prevents one from initializing a student from teacher weights, posing an additional technical challenge. We solve this challenge by adding a relatively lightweight score-matching pretraining stage before distillation (Sec.~\ref{subsec:from_scratch}), and demonstrating its necessity and efficiency via extensive experiments.

We validate our approaches by applying \ShortMethodName{} to distill the teacher into $4$ same-sized students using distribution matching and adversarial distillation procedures \citep{yin2024one, yin2024improved}. The resulting students collectively outperform single-student counterparts, setting new state-of-the-art FID scores of $\num{1.20}$ on one-step ImageNet-64$\times$64 generation (Tab.~\ref{tab:imagenet_short}) and \FIDSDADM{} on one-step zero-shot COCO2014 generation (Tab.~\ref{tab:sd_short}). We also distill the same teacher into $4$ smaller students, which achieve a competitive FID of \FIDIADMS{} on ImageNet (Tab.~\ref{tab:imagenet_short}), with $42\%$ less parameters per student. 
% \James{Critical take: while this result is good enough to include, I think it isn't hugely impressive. Showing some samples to help readers compare would be good. But only a 20\% increase is quite slim. Post-processing methods like quantization etc. can normally give a bigger runtime improvement for a smaller performance cost.} 
% \Weili{Provide a number for how much reduction in single-step generation time using smaller students.}.

We summarize our contributions below, which include:
\begin{itemize}
    \item A new framework, \ShortMethodName{}, that upgrades existing single-step diffusion distillation methods (Sec.~\ref{subsec:\ShortMethodName{}}) by increasing the effective model capacity without changing inference latency.
    \item Demonstrating the effectiveness of \ShortMethodName{} by training multiple same sized students using SOTA distillation techniques \citep{yin2024one, yin2024improved} in Sec.~\ref{subsec:\ShortMethodName{}-DMD}, resulting in new record FID scores in ImageNet-64$\times$64 (Sec.~\ref{subsec:imagenet}) and zero-shot text-to-image generation (Sec.~\ref{subsec:t2i}).
    \item A successful scheme to distill multiple smaller single-step students from the teacher model, achieving comparable generation quality with reduced inference time. 
    % \James{This was done in prior work already?}
    % opening new possibilities for faster generation.
\end{itemize}

==> sections/method.tex <==
\section{Method}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{plots/abstract_long_V2.pdf}
    % Link for image: https://nvidia-my.sharepoint.com/:p:/r/personal/yankes_nvidia_com/Documents/MSD_graph1.pptx?d=wd0da23f75bc94b3eb3e9fb32cfea7725&csf=1&web=1&e=voPtmP
    \caption{
        We visualize distilling into multiple students, where each student handles a subset of the input condition. At training, students are trained separately with filtered data. At inference, a single student is retrieved for generation given the corresponding input condition.
    }
    \label{fig:abstract_distill}
\end{figure}

In Sec.~\ref{subsec:\ShortMethodName{}}, we introduce the general \LongMethodName{} (\ShortMethodName{}) framework. In Sec.~\ref{subsec:\ShortMethodName{}-DMD}, we show how \ShortMethodName{} is applied to distribution matching and adversarial distillation. In Sec.~\ref{subsec:from_scratch}, we introduce an additional training stage enabling distilling into smaller students.

\begin{figure}[ht]
    \centering
    \vspace{-0.02\textheight}
    \includegraphics[trim={1.5cm 0cm 1.5cm 0cm}, width=0.8\linewidth]{plots/three_stage.pdf}
     % Link for image: https://nvidia-my.sharepoint.com/:p:/r/personal/yankes_nvidia_com/Documents/MSD_graph2.pptx?d=wfd499ba6b86f4ec6990467ddf21eedba&csf=1&web=1&e=I2XqXr
    \vspace{-0.025\textheight}
    \caption{
    Three-stage training scheme in Eq.~\ref{eqn:MSD-DMD-TSM}. Acronym meanings: {\blue \StageZeroName{}}: teacher score matching (Eq.~\ref{eqn:TSM} \& Eq.~\ref{eqn:MSD-DMD-TSM}); \customgreen{\StageOneName{}}: distribution matching (Eq.~\ref{eqn:MSD-DMD-TSM} \& Sec.~\ref{subsec:prelim_dm}); {\orange\StageTwoName{}}: adversarial distribution matching (Eq.~\ref{eqn:MSD-DMD-TSM} and Sec.~\ref{subsec:prelim_adm}). \customgreen{Stage 1} and {\orange Stage 2} are techniques from previous works that help with same-sized students; {\blue Stage 0} is our contribution, which is required for smaller students who cannot initialize with teacher weights.
    % \Jon{Looks great!  IMO seems a little confusing to have the one-step student change colors in stage-2.  What if you swapped the colors so the one-step student is red in stage1+2, and the "DM" is green and the "ADM" is orange? Also, can you make the cat images as big as possible in the pdf, since its a bit hard to tell difference between stage 1 and 2 cats, and you have spare vspace and hspace.}
        % \Jon{This figures makes it look like the output of the stage-0 model is fed as input the stage-1 model, is fed as input to the stage-2 model - maybe use a different notation to show "is initialized from" vs "input".  Also, it looks like the TSM cat is an input to the teacher and the DM/ADM cats could be outputs because their arrow comes in from the RHS.  Maybe easiest to have 3 separate blocks -- one for each stage -- and a frozen teacher in each block.  And connect the stages with the $\Distill$ notation perhaps.}
        % \Weili{I agree that it would be more clear to have 3 blocks and each block for a stage. Right now, it is hard to understand. }
    }
    \label{fig:three-stage_training}
    % \vspace{-0.01\textheight}
\end{figure}

\subsection{Distilling into multiple students}\label{subsec:\ShortMethodName{}}
We present \LongMethodName{} (\ShortMethodName), a general drop-in framework to be combined with any conditional single-step diffusion distillation method that enables a cheap upgrade of model capacity without impairing the inference speed. We first identify the key components of a single-step diffusion distillation framework and then present the modification of \ShortMethodName{}. 

In the vanilla one-student distillation, we have a pretrained teacher denoising diffusion model $\bmu_{\text{teacher}}$, a training dataset $\Data$, and a distillation method.
% \Jon{So, $\Distill_y$ is basically notation $G_{\textnormal{argmin}_{x} \mathcal{L}_y(x)}$?  Is this standard notation in some paper? I find it hard to parse in all the equations, as this notation hides what they are saying, and it forces you to hunt through the text to find this sentence.  IMO, I would drop this notation and expand the argmin if it fits in each equation. Or define exactly what this notation is with its own equation.  If the issue is that argmin is non-unique, or we don't actually reach it due to finite optimization, then I've seen people use the notation $\textnormal{Optimize}_x L_y (x)$, which feels more readable}
The distillation yields a single-step generator $\Generator(\bz;y\in \Label)$ via $\Generator = \Distill(\bmu_{\text{teacher}};\Data)$. The obtained generator $\Generator$ maps a random latent $\bz$ and an input condition $y$ into an image. 
% \Jon{Shapes seem non-standard.  Do you want the result of $\Distill$ to be parameters or a function? Using the parameters feels more standard to be, but I guess this saves you a bit of notation}
In comparison, in an \ShortMethodName{} scheme, we instead distill the teacher into $K$ different one-step generators $\{\Generator_k(\bz;y\in \Label_k)\}_{k=1}^K$ via 
\begin{equation}\label{eqn:MSD}
\Generator_k = \Distill(\mu_{\text{teacher}}, \Data_k = \Filter(\Data,\Label_k)),\ \ k=1,...,K
\end{equation}
Specifically, each distilled student $\Generator_k$ is specialized in handling a partitioned subset $\Label_k$ of the whole input condition set $\Label$. So, it is trained on a subset of the training data $\Data_k \subset \Data$, determined by $\Label_k$ via a filtering function $\Filter$. Fig.~\ref{fig:abstract_distill} illustrates this idea.

The partition of $\Label$ into $\{\Label_k\}_{k=1}^K$ determines the input condition groups for which each student is responsible. As a starting point, we make the following three simplifications for choosing a partition:
\begin{itemize}[leftmargin=*]
    \item \emph{Disjointness}: This prevents potential redundant training and redundant usage of model capacity.
    \item \emph{Equal size}: Since students have the same architecture, the partitions $\{\Label_k\}_{k=1}^K$ should be of equal size that require similar model capacity.
    \item \emph{Clustering}: Conditions within each partition should be more semantically similar than those in other partitions, so networks require less capacity to achieve a set quality on their partition.
\end{itemize}
The first two conditions can be easily satisfied in practice, while the third is not straightforward. For a class-conditional generation, partitioning by semantically similar and equal-sized classes serves a straightforward strategy, though extending it to text-conditional generation is nontrivial. Another promising strategy uses pretrained embedding layers such as the CLIP \citep{radford2021learning} embedding layer or the teacher embedding layer. 
One could find embeddings of the input conditions and then perform clustering on those embeddings, which are fixed-length numerical vectors containing implicit semantic information. We ablate partition strategies in Sec.~\ref{subsec:ablation}.

The data filtering function $\Filter$ determines the training subset data $\Data_k$ from $\Label_k$. For example, a vanilla filtering strategy could set $\Filter(\Data, \Label_k) =\Data_k:= \Data_{\Label_k}$, where $\Data_{\Label_k}$ denotes the subset of the training dataset $\Data$ that contains the desired condition $\Label_k$. Empirically, we found that this filtering works in most cases, although sometimes a different approach is justified, as demonstrated in Sec.~\ref{subsec:\ShortMethodName{}-DMD}.

\subsection{\ShortMethodName{} with distribution matching}\label{subsec:\ShortMethodName{}-DMD}
As a concrete example, we demonstrate the MSD framework using distribution matching (\StageOneName{}) and adversarial distillation techniques. Inspired by the two-stage framework in \cite{yin2024improved}, each of our students is trained with a distribution matching  scheme at the first stage and finetuned with an additional adversarial loss at the second stage (adversarial distribution matching, or \StageTwoName{}):
\begin{equation}\label{eqn:MSD-DMD}
\begin{aligned}
\Generator_k^{(1)} &= \Distill_{\StageOneName}\left(\bmu_{\text{teacher}}, \Filter_{\StageOneName}(\Data_{\StageOneName},\Label_k)\right),\ \ k=1,...,K,\\
\Generator_k^{(2)} &= \Distill_{\StageTwoName}\left(\bmu_{\text{teacher}}, \Filter_{\StageTwoName}(\Data_{\StageTwoName},\Label_k);\Generator_k^{(1)}\right),\ \ k=1,...,K,
\end{aligned}    
\end{equation}
where we recall that $\bmu_{\text{teacher}}$ is the teacher diffusion model, $\Generator_k^{(i)}$ is the $k$-th student generator at the $i$-th stage, $\Filter$ is the data filtering function, $\Data$ is the training data, and $\Label_k$ is the set of labels that student $k$ is responsible of. The first stage $\Distill_{\StageOneName}$ uses distribution matching with either a complemented regression loss or the TTUR, with details in Sec.~\ref{subsec:prelim_dm}. These two methods achieve optimal training efficiency among other best-performing single-step distillation methods \citep{xie2024distillation, zhou2024score, kim2023consistency} without an adversarial loss, with a detailed comparison in App.~\ref{sec:first_stage_comparison}. The second stage $\Distill_{\StageTwoName}$ adds an additional adversarial loss (details in Sec.~\ref{subsec:prelim_adm}, which introduces minimal additional computational overhead and allows resuming from the first stage checkpoint, making it a natural choice.

\paragraph{Designing the training data} From Sec.~\ref{sec:prelim}, the data required for \StageOneName{} and \StageTwoName{} are $\Data_{\StageOneName} = (\Data_{\text{paired}},\mcl{C})$ and $\Data_{\StageTwoName} = (\Data_{\text{real}},\mcl{C})$, where $\Data_{\text{paired}},\Data_{\text{real}},\mcl{C}$ represents generated paired data, real data and separate conditional input, respectively. We now discuss choices for the filtering function.

For the first stage data filtering $\Filter_{\StageOneName}$, we propose $\Filter_{\StageOneName}(\Data_{\StageOneName},\Label_k) = (\Data_{\text{paired}}, \mcl{C}_{\Label_k})$, where $\mcl{C}_{\Label_k}$ denotes the subset of condition inputs $\mcl{C}$ that contains $\Label_k$. In other words, we sample all input conditions only on the desired partition for the KL loss but use the whole paired dataset for the regression loss. This special filtering is based on the observation that the size of $\Data_{\text{paired}}$ critically affects the terminal performance of DMD distillation: using fewer pairs causes mode collapse, whereas using more pairs challenge the model capacity. Na\"ively filtering paired datasets by partition reduces the paired dataset size for each student and leads to worse performance, as in our ablation in App.~\ref{subsec:paired_size_ablation}. Instead of generating more paired data to mitigate this imbalance, we simply reuse the original paired dataset for the regression loss. This is remarkably effective, which we hypothesize is because paired data from other input conditions provides effective gradient updates to the shared weights in the network.

% We attribute such effectiveness to the fact that each student network is forced to cover the same modes for regression loss, thereby maintaining the shape of its output distribution, meanwhile allowing it to focus on a subset partition for VSD loss, obtaining better score estimation for a subset of modes.

For the second stage, we stick to the simple data filtering $\Filter_{\StageTwoName}(\Data_{\StageTwoName},\Label_k) = (\Data_{\text{real},\Label_k}, \mcl{C}_{\Label_k})$, so that both adversarial and KL losses focus on the corresponding partition, given that each student has enough mode coverage from the first stage.

\subsection{Distilling smaller students from scratch}\label{subsec:from_scratch}
Via the frameworks presented in the last two sections, \ShortMethodName{} enables a performance upgrade over alternatives for one student with the same model architecture. In this section, we investigate training multiple students with smaller architectures -- and thus faster inference time -- without impairing much performance.
However, this requires distilling into a student with a different architecture, preventing initialization from pretrained teacher weights. Distilling a single-step student from scratch has previously been difficult \citep{xie2024distillation}, and we could not obtain competitive results with the simple pipeline in Eq.~\ref{eqn:MSD-DMD}. Therefore, we propose an additional pretraining phase $\Distill_\StageZeroName$, with \StageZeroName{} denoting Teacher Score Matching, to find a good initialization for single-step distillation. \StageZeroName{} employs the following score-matching loss:
\begin{equation}\label{eqn:TSM}
\mcl{L}_{\StageZeroName} = \E_t[\StageZeroWeight \|\bmu_{\StageZeroName}^\varphi(\bx_t,t) - \bmu_{\text{teacher}}(\bx_t,t)\|_2^2],
\end{equation}
where the smaller student with weights $\varphi$ is trained to match the teacher's score on real images at different noise levels. This step provides useful initialization weights for single-step distillation and is crucial to ensure convergence. With \StageZeroName{} added, the whole pipeline now becomes:
\begin{equation}\label{eqn:MSD-DMD-TSM}
\begin{aligned}
\bmu^{(0)} &= \Distill_{\text{TSM}}\left(\bmu_{\text{teacher}}, \Data_{\text{real}}\right),\\
\Generator_k^{(1)} &= \Distill_{\StageOneName}\left(\bmu_{\text{teacher}}, \Filter_{\StageOneName}(\Data_{\StageOneName},\Label_k);\bmu^{(0)}\right),\ \ k=1,...,K,\\
\Generator_k^{(2)} &= \Distill_{\StageTwoName}\left(\bmu_{\text{teacher}}, \Filter_{\StageTwoName}(\Data_{\StageTwoName},\Label_k);\Generator_k^{(1)}\right),\ \ k=1,...,K.
\end{aligned}    
\end{equation}
Although a smaller student may not perfectly match the teacher's score, it still provides a good initialization for stages 1 and 2. The performance gap is remedied in the latter stages by focusing on a smaller partition for each student. This three-stage training scheme is illustrated in Fig.~\ref{fig:three-stage_training}.

% \Jon{
% I think our paper could use a figure to illustrate this setup.
% So, some kind of figure, expanding on the "training" block in Figure 1.
% This could look like "Stage 0" on the left, "Stage 1" in the middle, and "Stage 2" on the right—or whatever you think is best.
% Then, we use this figure to describe to the reader the difference between identical student and different-sized student training methods.
% }

==> sections/prelims.tex <==
\section{Preliminary}\label{sec:prelim}
We introduce the background on diffusion models in Sec.~\ref{subsec:prelim_diffusion} and distribution matching distillation (DMD) in Sec.~\ref{subsec:prelim_dm}. We discuss how applying adversarial losses to improve distillation in Sec.~\ref{subsec:prelim_adm}.

\subsection{Diffusion Models}\label{subsec:prelim_diffusion}
Diffusion models learn to generate data by estimating the score functions \citep{song2020score} of the corrupted data distribution on different noise levels. Specifically, at different timesteps $t$, the data distribution $p_{\text{real}}$ is corrupted with an independent Gaussian noise: $p_{t,\text{real}}(\bx_t) = \int p_{\text{real}}(\bx)q_t(\bx_t|\bx)d\bx$ where $q_t(\bx_t|\bx) \sim \mcn(\alpha_t \bx,\sigma_t^2 \bI)$ with predetermined $\alpha_t,\sigma_t$ following a forward diffusion process~\citep{song2020score,ho2020denoising}. 
The neural network learns the score of corrupted data $\bs_{\text{real}} := \nabla_{\bx_t} \log p_{t,\text{real}}(\bx_t)= -(\bx_t-\alpha_t \bx) / \sigma_t^2$ by equivalently predicting the denoised $\bx$: $\bmu(\bx_t,t) \approx \bx$. After training with the denoising score matching loss $\E_{\bx,t,\bx_t}[\lambda_t \|\bmu(\bx_t,t)-\bx\|_2^2]$, where $\lambda_t$ is a weighting cofficient,
% \Weili{It is good to define the denoising loss here}
the model generates the data by an iterative denoising process over a decreasing sequence of time steps.
% \Jon{Use bm for vectors? Ex., $x_t \to \bm{x}_t, \mu \to \bm{\mu}, s \to \bm{s}, \dots$.  Easy to do if replace all occurrences of $x_t$ with a command, then make command use bold}
% \Yanke{Edited}

\subsection{Distribution Matching Distillation}\label{subsec:prelim_dm}
Inspired by \citet{wang2024prolificdreamer}, the works of \citet{luo2024diff, yin2024one, ye2024score, nguyen2024swiftbrush} aim to train the single-step distilled student to match the generated distribution of the teacher diffusion model. This is done by minimizing the following reverse KL divergence between teacher and student output distributions, diffused at different noise levels for better support over the ambient space:
\begin{equation}\label{eqn:KL}
\begin{aligned}
\E_t D_{\text{KL}}(p_{t,\text{fake}} \| p_{t,\text{real}})=\E_{\bx_t} \left( \log \left( \frac{p_{t,\text{fake}}(\bx_t)}{p_{t,\text{real}}(\bx_t)} \right) \right).
\end{aligned}
\end{equation}
The training only requires the gradient of Eq.~\eqref{eqn:KL}, which reads (with a custom weighting $w_t$):
\begin{equation}\label{eqn:KL_gradient}
\begin{aligned}
\nabla_\theta \mathcal{L}_{\text{KL}}(\theta) := \nabla_\theta \E_t D_{\text{KL}} \simeq \E_{\bz,t,\bx_t}[w_t\alpha_t(\bs_{\text{fake}}(\bx_t,t) - \bs_{\text{real}}(\bx_t,t)) \nabla_\theta G_\theta(\bz)],
\end{aligned}
\end{equation}
where $\bz\sim \mcn(0,\bI), t\sim \text{Uniform}[T_{\min},T_{\max}]$, and $\bx_t \sim q(\bx_t|\bx)$, the noise injected version of $\bx = G_\theta(\bz)$ generated by the one-step student. Here, we assume the teacher denoising model accurately approximates the score of the real data, and a ``fake'' denoising model approximates the score of generated fake data:
\begin{equation}\label{eqn:score_estimation}
\bs_{\text{real}}(\bx_t,t) \approx -\frac{\bx_t - \alpha_t \bmu_{\text{teacher}}(\bx_t,t)}{\sigma_t^2}, \ \ \bs_{\text{fake}}(\bx_t,t) \approx -\frac{\bx_t - \alpha_t \bmu_{\text{fake}}(\bx_t,t)}{\sigma_t^2}.
\end{equation}
The ``fake'' denoising model is trained with the denoising objective with weighting $\lambda_t$:
\begin{equation}\label{eqn:fakescore_denoising}
\mcl{L}_{\text{denoise}}(\phi) = \E_{\bz,t,\bx_t}[\lambda_t\|\bmu_{\text{fake}}^\phi(\bx_t,t) - \bx\|_2^2].
\end{equation}
The generator and the ``fake'' denoising model are updated alternatively. To facilitate better convergence of the KL divergence, Distribution Matching Distillation (DMD) and DMD2 \citep{yin2024improved} used two distinct strategies, both significantly improving the generation performance. DMD proposes to complement the KL loss with a regression loss to encourage mode covering:
\begin{equation}\label{eqn:reg_loss}
\mcl{L}_{\text{reg}}(\theta) = \E_{(\bz,y)\sim \mcl{D}_{\text{paired}}} \ell (G_\theta(\bz),y),
\end{equation}
where $\mcl{D}_{\text{paired}}$ is a dataset of latent-image pairs generated by the teacher model offline, and $\ell$ is the Learned Perceptual Image Patch Similarity (LPIPS) \citep{zhang2018unreasonable}. 
DMD2 instead applies a two-timescale update rule (TTUR), where they update the ``fake'' score model for $N$ steps per generator update, allowing more stable convergence. We use distribution matching (\StageOneName{}) to refer to all relevant techniques introduced in this section.

% \Jon{This section is notationally dense, but much of it is not in the glossary. Some terms that I don't see defined there: $t, p_{t, \cdot}, q, x_t, w_t, \alpha_t, s_{\cdot}, \theta, z, \lambda_t, T_{\cdot}, \mu_{\cdot}, \sigma_t, \mcl{L}_{\cdot}, \ell, \phi, y$.  For any notation that is only used in this section -- consider if its even worth introducing notation just to use it once.}\Yanke{Will make this decision later}

\subsection{Enhancing distillation quality with adversarial loss}\label{subsec:prelim_adm}
The adversarial loss, originally proposed by \citet{goodfellow2020generative}, has shown a remarkable capability in diffusion distillation to enhance sharpness and realism in generated images, thus improving generation quality. Specifically, DMD2 \citep{yin2024improved} proposes adding a minimal discriminator head to the bottleneck layer of the ``fake'' denoising model $\mu_{\text{fake}}$, which is naturally compatible with DMD's alternating training scheme and the TTUR. Moreover, they showed that one should first train the model without GAN to convergence, then add the GAN loss and continue training. This yields better terminal performance than training with the GAN loss from the beginning.
We use adversarial distribution matching (\StageTwoName{}) to refer to distribution matching with added adversarial loss.

% Both the TTUR and the added adversarial loss are proposed in the DMD2 paper. To avoid notational confusion, we use distribution matching (\StageOneName{}) to refer to relevant techniques without the adversarial loss (i.e., the added regression loss and TTUR), and we use adversarial distribution matching (\StageTwoName{}) to refer to the added adversarial loss specifically.

% \James{We discuss this in related work too. I think we can probably remove this section if we need space.}

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
\textbf{Diffusion Sampling Acceleration. }
% \Yanke{Trying to be concise here as our idea is kind of orthogonal. Can be more elaborative}
While a line of work aims to accelerate diffusion models via fast numerical solvers for the PF-ODE \citep{lu2022dpm,lu2022dpmp,zheng2024dpm,karras2022elucidating,liu2022pseudo}, they usually still require more than $10$ steps. Training-based methods that usually follow the knowledge distillation pipeline can achieve low-step or even one-step generation. 
\citet{luhman2021knowledge} first used the diffusion model to generate a noise and image pair dataset that is then used to train a single-step generator. DSNO \citep{zheng2023fast} precomputes the denoising trajectory and uses neural operators to estimate the whole PF-ODE path. Progressive distillation \citep{salimans2022progressive, meng2023distillation} iteratively halves the number of sampling steps required without needing an offline dataset. Rectified Flow \citep{liu2022flow} and follow-up works \citep{liu2023instaflow, yan2024perflow} straighten the denoising trajectories to allow sampling in fewer steps. Another approach uses self-consistent properties of denoising trajectories to inject additional regularization for distillation \citep{gu2023boot, berthelot2023tract, song2023consistency, song2023improved, luo2023lcm, ren2024hyper, kim2023consistency}. 

The methods above require the student to follow the teacher's trajectories.
% \James{Removed ``have sub-optimal performance since''. I feel this is hard to say definitively.}
Instead, 
% inspired by the VSD loss first proposed in 3D generation \citep{wang2024prolificdreamer}, 
a recent line of works aims to only match the distribution of the student and teacher output via variational score distillation \citep{yin2024one, yin2024improved, salimans2024multistep, xie2024distillation, luo2024diff, zhou2024score, nguyen2024swiftbrush}. The adversarial loss \citep{goodfellow2020generative}, often combined with the above techniques, has been used to enhance the distillation performance further \citep{xiao2021tackling, zheng2024diffusion, sauer2023adversarial, sauer2024fast, wang2022diffusion, xu2024ufogen, lin2024sdxl, kim2023consistency}. Although \ShortMethodName{} is conceptually compatible and offers a performance boost to all of these distillation methods, in this work, we demonstrate two specific techniques: distribution matching \citep{yin2024one} and adversarial distillation \citep{yin2024improved}.

\textbf{Mixture of experts training and distillation. }
Mixture of Experts (MoE), first proposed in \cite{jordan1994hierarchical}, has found success in training very large-scale neural networks \citep{shazeer2017outrageously, lepikhin2020gshard, fedus2022switch, lewis2021base, borde2024breaking}. Distilling a teacher model into multiple students was explored by \citet{hinton2015distilling}, and after that, has been further developed for supervised learning \citep{chen2020online, ni2023knowledge, chang2022one} and language modeling \citep{xie2024mode, kudugunta2021beyond, zuo2022moebert}. Although several works \citep{hoang2018mgan, park2018megan, ahmetouglu2021hierarchical} have proposed MoE training schemes for generative adversarial networks, they train the MoE from scratch. This requires carefully tuning the multi-expert adversarial losses. eDiff-I \citep{balaji2022ediff} uses different experts in different denoising timesteps for a multi-step diffusion model. A recent work \citep{zhou2024variational} proposes to distill a pretrained diffusion model into an MoE for policy learning, which shares similar motivations with our work. However, to the best of our knowledge, \ShortMethodName{} is the first method to \textit{distill} multi-step teacher diffusion models into multiple one-step students for image generation.

% In a predictive mixture-of-experts model, multiple experts are trained to specialize in specific data segments. A routing mechanism such as a gating layer is employed to direct input to relevant experts, and their (soft) prediction outputs are aggregated. Conditional generative models, in comparison, have quite different schemes. Since generated outputs do not admit simple aggregation, only one student is used at inference time. However, on the input front, the condition information admits simple routing strategies, such as class-based partitioning or clustering in the embedding space.

 

\textbf{Efficient architectures for diffusion models. } In addition to reducing steps, an orthogonal approach aims to accelerate diffusion models with more efficient architectures. A series of works \citep{bao2022all, peebles2023scalable, hoogeboom2023simple} introduces vision transformers to diffusion blocks and trains the diffusion model with new architectures from scratch. Another line of work selectively removes or modifies certain components of a pretrained diffusion model and then either finetunes \citep{kim2023architectural, li2024snapfusion, zhang2024laptop} or re-trains \citep{zhao2023mobilediffusion} the lightweight diffusion model, from which step-distillation can be further applied \citep{li2024snapfusion, zhao2023mobilediffusion}. Our approach is orthogonal to these works in two regards: 1) In our method, each student only handles a subset of data, providing a gain in relative capacity. 2) Instead of obtaining a full diffusion model, our method employs a lightweight pretraining stage to obtain a good initialization for single-step distillation. Combining MSD with more efficient architectures is a promising future direction.
